The Degenerate Principal Series Representations of Exceptional Groups of Type $E_7$ over $p$-adic Fields

In this paper, we study the degenerate principal series of a split, simply-connected, simple p-adic group of type $E_7$. We determine the points of reducibility and the maximal semi-simple subrepresentation at each point.

==> E7regular_table.tex <==
\begin{itemize}
\item For $\para{P}=\para{P}_1$
\begin{table}[H]
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|} \hline
\diagbox{$ord\bk{\chi}$}{$s$} & $ -\frac{17}{2} $ & $ -\frac{15}{2} $ & $ -\frac{13}{2} $ & $ -\frac{11}{2} $ & $ -\frac{9}{2} $ & $ -\frac{7}{2} $ & $ -\frac{5}{2} $ & $ -\frac{3}{2} $ & $ -\frac{1}{2} $ & $ 0 $ \\ \hline \hline
$1$ &  \makecell{reg. \\ red.} &  \makecell{non-reg. \\ irr.} &  \makecell{non-reg. \\ irr.} &  \makecell{reg. \\ red.} &  \makecell{non-reg. \\ irr.} &  \makecell{reg. \\ red.} &  \makecell{non-reg. \\ irr.} &  \makecell{non-reg. \\ irr.} &  \makecell{reg. \\ red.} &  \makecell{non-reg. \\ irr.} \\ \hline
$2$ &  \makecell{reg. \\ irr.} &  \makecell{reg. \\ irr.} &  \makecell{reg. \\ irr.} &  \makecell{reg. \\ irr.} &  \makecell{reg. \\ irr.} &  \makecell{reg. \\ irr.} &  \makecell{reg. \\ irr.} &  \makecell{reg. \\ irr.} &  \makecell{reg. \\ red.} &  \makecell{non-reg. \\ irr.} \\ \hline
\end{tabular}
 %\caption{$P=P_1$} %\notableentry 
\label{Tab::E7::REG::P_1}
 \end{table}

\item For $\para{P}=\para{P}_2$
\begin{table}[H]
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|} \hline
\diagbox{$ord\bk{\chi}$}{$s$} & $ -7 $ & $ -6 $ & $ -5 $ & $ -4 $ & $ -3 $ & $ -2 $ & $ -\frac{3}{2} $ & $ -1 $ & $ -\frac{1}{2} $ & $ 0 $ \\ \hline \hline
$1$ &  \makecell{reg. \\ red.} &  \makecell{non-reg. \\ irr.} &  \makecell{reg. \\ red.} &  \makecell{reg. \\ red.} &  \makecell{reg. \\ red.} &  \makecell{reg. \\ red.} &  \makecell{non-reg. \\ irr.} &  \makecell{reg. \\ red.} &  \makecell{non-reg. \\ irr.} &  \makecell{non-reg. \\ irr.} \\ \hline
$2$ &  \makecell{reg. \\ irr.} &  \makecell{reg. \\ irr.} &  \makecell{reg. \\ irr.} &  \makecell{reg. \\ irr.} &  \makecell{reg. \\ irr.} &  \makecell{reg. \\ red.} &  \makecell{non-reg. \\ irr.} &  \makecell{non-reg. \\ irr.} &  \makecell{non-reg. \\ irr.} & \color{red}{unknown} \\ \hline
\end{tabular}
 %\caption{$P=P_1$} %\notableentry 
\label{Tab::E7::REG::P_2}
 \end{table}
\newpage
\item For $\para{P}=\para{P}_3$
\begin{table}[H]
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|} \hline
\diagbox{$ord\bk{\chi}$}{$s$} & $ -\frac{11}{2} $ & $ -\frac{9}{2} $ & $ -\frac{7}{2} $ & $ -\frac{5}{2} $ & $ -2 $ & $ -\frac{3}{2} $ & $ -1 $ & $ -\frac{1}{2} $ & $ -\frac{1}{6} $ & $ 0 $ \\ \hline \hline
$1$ &  \makecell{reg. \\ red.} &  \makecell{reg. \\ red.} &  \makecell{reg. \\ red.} &  \makecell{reg. \\ red.} &  \makecell{non-reg. \\ irr.} &  \makecell{reg. \\ red.} &  \makecell{non-reg. \\ irr.} &  \makecell{reg. \\ red.} &  \makecell{non-reg. \\ irr.} &  \makecell{non-reg. \\ irr.} \\ \hline
$2$ &  \makecell{reg. \\ irr.} &  \makecell{reg. \\ irr.} &  \makecell{reg. \\ irr.} &  \makecell{reg. \\ red.} &  \makecell{non-reg. \\ irr.} &  \makecell{reg. \\ red.} &  \makecell{non-reg. \\ irr.} &  \makecell{reg. \\ red.} &  \makecell{reg. \\ irr.} &  \makecell{non-reg. \\ irr.} \\ \hline
$3$ &  \makecell{reg. \\ irr.} &  \makecell{reg. \\ irr.} &  \makecell{reg. \\ irr.} &  \makecell{reg. \\ irr.} &  \makecell{reg. \\ irr.} &  \makecell{reg. \\ irr.} &  \makecell{reg. \\ irr.} &  \makecell{reg. \\ red.} &  \makecell{non-reg. \\ irr.} &  \makecell{reg. \\ irr.} \\ \hline
\end{tabular}
 %\caption{$P=P_1$} %\notableentry 
\label{Tab::E7::REG::P_3}
 \end{table}
\item For $\para{P}=\para{P}_4$
\begin{table}[H]
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|} \hline
\diagbox{$ord\bk{\chi}$}{$s$} & $ -4 $ & $ -3 $ & $ -2 $ & $ -\frac{3}{2} $ & $ -1 $ & $ -\frac{2}{3} $ & $ -\frac{1}{2} $ & $ -\frac{1}{3} $ & $ -\frac{1}{4} $ & $ 0 $ \\ \hline \hline
$1$ &  \makecell{reg. \\ red.} &  \makecell{reg. \\ red.} &  \makecell{reg. \\ red.} &  \makecell{reg. \\ red.} &  \makecell{reg. \\ red.} &  \makecell{reg. \\ red.} &  \makecell{reg. \\ red.} &  \makecell{non-reg. \\ irr.} &  \makecell{non-reg. \\ irr.} & \color{red}{unknown} \\ \hline
$2$ &  \makecell{reg. \\ irr.} &  \makecell{reg. \\ irr.} &  \makecell{reg. \\ red.} &  \makecell{reg. \\ red.} &  \makecell{reg. \\ red.} &  \makecell{reg. \\ irr.} &  \makecell{reg. \\ red.} &  \makecell{reg. \\ irr.} &  \makecell{non-reg. \\ irr.} &  \makecell{reg. \\ red.} \\ \hline
$3$ &  \makecell{reg. \\ irr.} &  \makecell{reg. \\ irr.} &  \makecell{reg. \\ irr.} &  \makecell{reg. \\ irr.} &  \makecell{reg. \\ red.} &  \makecell{reg. \\ red.} &  \makecell{reg. \\ irr.} &  \makecell{non-reg. \\ irr.} &  \makecell{reg. \\ irr.} &  \makecell{non-reg. \\ irr.} \\ \hline
$4$ &  \makecell{reg. \\ irr.} &  \makecell{reg. \\ irr.} &  \makecell{reg. \\ irr.} &  \makecell{reg. \\ irr.} &  \makecell{reg. \\ irr.} &  \makecell{reg. \\ irr.} &  \makecell{reg. \\ red.} &  \makecell{reg. \\ irr.} &  \makecell{non-reg. \\ irr.} &  \makecell{non-reg. \\ irr.} \\ \hline
\end{tabular}
 %\caption{$P=P_1$} %\notableentry 
\label{Tab::E7::REG::P_4}
 \end{table}
\item For $\para{P}=\para{P}_5$
\begin{table}[H]
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|} \hline
\diagbox{$ord\bk{\chi}$}{$s$} & $ -5 $ & $ -4 $ & $ -3 $ & $ -2 $ & $ -\frac{3}{2} $ & $ -1 $ & $ -\frac{2}{3} $ & $ -\frac{1}{2} $ & $ -\frac{1}{3} $ & $ 0 $ \\ \hline \hline
$1$ &  \makecell{reg. \\ red.} &  \makecell{reg. \\ red.} &  \makecell{reg. \\ red.} &  \makecell{reg. \\ red.} &  \makecell{reg. \\ red.} &  \makecell{reg. \\ red.} &  \makecell{non-reg. \\ irr.} &  \makecell{non-reg. \\ irr.} &  \makecell{non-reg. \\ irr.} & \makecell{non-reg. \\ irr.} \\ \hline
$2$ &  \makecell{reg. \\ irr.} &  \makecell{reg. \\ irr.} &  \makecell{reg. \\ irr.} &  \makecell{reg. \\ red.} &  \makecell{reg. \\ red.} &  \makecell{reg. \\ red.} &  \makecell{reg. \\ irr.} &  \makecell{non-reg. \\ irr.} &  \makecell{reg. \\ irr.} & \color{red}{unknown} \\ \hline
$3$ &  \makecell{reg. \\ irr.} &  \makecell{reg. \\ irr.} &  \makecell{reg. \\ irr.} &  \makecell{reg. \\ irr.} &  \makecell{reg. \\ irr.} &  \makecell{reg. \\ red.} &  \makecell{non-reg. \\ irr.} &  \makecell{reg. \\ irr.} &  \makecell{non-reg. \\ irr.} &  \makecell{non-reg. \\ irr.} \\ \hline
\end{tabular}
 %\caption{$P=P_1$} %\notableentry 
\label{Tab::E7::REG::P_5}
 \end{table}
\item For $\para{P}=\para{P}_6$
\begin{table}[H]
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|} \hline
\diagbox{$ord\bk{\chi}$}{$s$} & $ -\frac{13}{2} $ & $ -\frac{11}{2} $ & $ -\frac{9}{2} $ & $ -\frac{7}{2} $ & $ -\frac{5}{2} $ & $ -2 $ & $ -\frac{3}{2} $ & $ -1 $ & $ -\frac{1}{2} $ & $ 0 $ \\ \hline \hline
$1$ &  \makecell{reg. \\ red.} &  \makecell{reg. \\ red.} &  \makecell{non-reg. \\ irr.} &  \makecell{reg. \\ red.} &  \makecell{reg. \\ red.} &  \makecell{non-reg. \\ irr.} &  \makecell{non-reg. \\ irr.} &  \makecell{non-reg. \\ irr.} &  \makecell{reg. \\ red.} &  \makecell{non-reg. \\ irr.} \\ \hline
$2$ &  \makecell{reg. \\ irr.} &  \makecell{reg. \\ irr.} &  \makecell{reg. \\ irr.} &  \makecell{reg. \\ irr.} &  \makecell{reg. \\ red.} &  \makecell{non-reg. \\ irr.} &  \makecell{non-reg. \\ irr.} &  \makecell{non-reg. \\ irr.} &  \makecell{reg. \\ red.} &  \makecell{non-reg. \\ irr.} \\ \hline
\end{tabular}
 %\caption{$P=P_1$} %\notableentry 
\label{Tab::E7::REG::P_6}
 \end{table}
\newpage
\item For $\para{P}=\para{P}_7$
\begin{table}[H]
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|} \hline
\diagbox{$ord\bk{\chi}$}{$s$} & $ -9 $ & $ -8 $ & $ -7 $ & $ -6 $ & $ -5 $ & $ -4 $ & $ -3 $ & $ -2 $ & $ -1 $ & $ 0 $ \\ \hline \hline
$1$ &  \makecell{reg. \\ red.} &  \makecell{non-reg. \\ irr.} &  \makecell{non-reg. \\ irr.} &  \makecell{non-reg. \\ irr.} &  \makecell{reg. \\ red.} &  \makecell{non-reg. \\ irr.} &  \makecell{non-reg. \\ irr.} &  \makecell{non-reg. \\ irr.} &  \makecell{reg. \\ red.} &  \makecell{non-reg. \\ irr.} \\ \hline
$2$ &  \makecell{reg. \\ irr.} &  \makecell{reg. \\ irr.} &  \makecell{reg. \\ irr.} &  \makecell{reg. \\ irr.} &  \makecell{reg. \\ irr.} &  \makecell{reg. \\ irr.} &  \makecell{reg. \\ irr.} &  \makecell{reg. \\ irr.} &  \makecell{reg. \\ irr.} & \color{red}{unknown} \\ \hline
\end{tabular}
 %\caption{$P=P_1$} %\notableentry 
\label{Tab::E7::REG::P_7}
 \end{table}

